DeepMAD: Mathematical Architecture Design for Deep Convolutional Neural Network

The rapid advances in Vision Transformer (ViT) refresh the state-of-the-art performances in various vision tasks, overshadowing the conventional CNN-based models. This ignites a few recent striking-back research in the CNN world showing that pure CNN models can achieve as good performance as ViT models when carefully tuned. While encouraging, designing such high-performance CNN models is challenging, requiring non-trivial prior knowledge of network design. To this end, a novel framework termed Mathematical Architecture Design for Deep CNN (DeepMAD) is proposed to design high-performance CNN models in a principled way. In DeepMAD, a CNN network is modeled as an information processing system whose expressiveness and effectiveness can be analytically formulated by their structural parameters. Then a constrained mathematical programming (MP) problem is proposed to optimize these structural parameters. The MP problem can be easily solved by off-the-shelf MP solvers on CPUs with a small memory footprint. In addition, DeepMAD is a pure mathematical framework: no GPU or training data is required during network design. The superiority of DeepMAD is validated on multiple large-scale computer vision benchmark datasets. Notably on ImageNet-1k, only using conventional convolutional layers, DeepMAD achieves 0.7% and 1.5% higher top-1 accuracy than ConvNeXt and Swin on Tiny level, and 0.8% and 0.9% higher on Small level.

==> xiachen/1_introduction_xiachen.tex <==





%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figure/first_blood.jpg}
  \caption{
  \textbf{ImageNet-1K classification} results for Deep-MAD and other state-of-the-art works.
  Each bubble's area is proportional to the GFLOPs of the model.
  \todo{We demonstrate that the, with pure convolutional structures, the proposed Deep-MAD method can achieve better performance than those ViT or ViT-inspired models with smaller model size and less computation cost.}
  }
  \label{fig:first_blood}
\end{figure}

%----- VIT replaces CNN ------
Convolutional neural networks (CNN) have been the predominant models in computer vision in the past decades~\cite{ka2012deepcnn, efficientnet, xie2016aggregated}.
% The innovation of residual link~\cite{He2015resnet} and batch normalization~(BN)~\cite{si2015batchnorm} scales CNN models up to a few thousand layers, outperforming previous non-deep learning methods.
% For a very long time, the CNN-based backbone has been a prevalent paradigm in most tasks.
Until recently, the emergence of Vision Transformer (ViT)~\cite{dosovitskiy2020vit, deit2021, liu2021swin} establishes a novel paradigm that surpasses CNN models in large-scale datasets~\cite{imagenet, cocodataset}. The ViT introduces self-attention~\cite{attention2017} mechanism as well as other dedicated components such as LayerNorm~\cite{layernorm}, non-overlapping token patching~\cite{dosovitskiy2020vit, deit2021, liu2021swin} and positional embedding~\cite{dosovitskiy2020vit}. Equipped with these novel building blocks, ViT outperforms CNN models and becomes one of the most popular models in the computer vision community.

%----- CNN is still useful because well-supported on hardware
Albeit very successful, ViT is not yet a perfect universal deep learning model for all tasks. The original self-attention layer in ViT requires quadratic computational complexity in token size~\cite{mehta2021mobilevit}. The training of ViT is more difficult than CNN. For example, most ViT models cannot converge well using SGD optimizer~\cite{deit2021, dosovitskiy2020vit}. When the training set is too small, ViT may not generalize as well as CNN~\cite{liu2022convnet}. On the other hand, CNN models enjoy several merits over ViT models. First, CNN has been highly optimized on various hardware platforms and is well-supported by literally every deep learning framework. Second, CNN is easier to train and converges well when using either SGD or Adam~\cite{He2015resnet, liu2022convnet, ka2012deepcnn, efficientnet, xie2016aggregated} optimizer. Third, CNN has strong theoretical guarantees. For example, deep CNN is proved to be a universal approximator for any smooth functions~\cite{chan2021redunet, regnet2020}. The complexity and trainability of CNN have been extensively studied in literature~\cite{regnet2020, ka2012deepcnn, xie2016aggregated}, meaning that its learning power is backed up by the deep learning theories~\cite{principlesofdeeplearning-2022, chan2021redunet}.

% CNN strikes back, using ViT-inspired designs
Considering the decades of efforts devoted to the development of CNN models, it would be a great waste if we throw away all CNN models together with all existing deep learning theories built upon them. A few recent researches try to revive CNN models using novel architecture designs \cite{yu2022metaformer,heo2021pit,liu2022convnet,ding2022scaling,yu2022metaformer}. While these efforts abridged the gap between pure CNN models and ViT models, designing such high-performance CNN models is challenging. Most methods borrow ViT components into CNN models, such as replacing the attention matrix with a convolutional counterpart and/or keeping the macrostructure of ViT, including LayerNorm and fully connected layer. The optimizer is also switched from the conventional SGD to Adam as in ViT. After modifications, the new CNN backbones are considerably different from the conventional ResNet-like CNN models. Therefore, it is important for us to figure out whether these ViT-like modifications are essential in the next-generation CNN models and whether the pure CNN models can exceed the transformer-based models and transformer-like (CNN) models.

% \todo{move below to Related Work}
% For example, MetaFormer~\cite{yu2022metaformer} shows that the attention matrix in ViT can be replaced by pooling layer; PiT~\cite{heo2021pit} adopts pooling between transformer blocks for the spatial dimension reduction to achieve better performance, which is inspired by the effect of pooling operation in CNNs; ConvNext~\cite{liu2022convnet} mimics the transformer layer using depth-wise convolution and use the same macro backbone design as Swin Transformer~\cite{liu2021swin}; RepLKNet~\cite{ding2022scaling} scales up the kernels beyond 31x31 to capture global Receptive Fields as attention. All these efforts demonstrated that CNN models can achieve as good performance as ViT models when tuned carefully.
% % xuan: add PiT and RepLKNet
% \todo{move above to Related Work}

% Can we do better, mathematically


In this work, we move one more step in this direction. We show that the potential of the conventional Conv+BN+ReLU paradigm is greatly under-estimated. \textbf{We do not need any above CNN ``modernizations'' at all to make CNN great again}. To this end, we propose a novel design paradigm termed \textbf{Deep-MAD} where MAD is short for \textit{Mathematical Architecture Design}. Deep-MAD is built upon the recent advances of deep learning theories~\cite{principlesofdeeplearning-2022, chan2021redunet, regnet2020}. To optimize the architecture of CNN models, Deep-MAD innovates a constrained mathematical programming (MP) problem whose solution reveals the optimized structural parameters, such as the widths and depths of the network. Particularly, the Deep-MAD maximizes the differential entropy~\cite{zhenhong2022maedet, sk1997entropy, yy2020entropy, etj1957entropy} of the network \todo{with constrained effectiveness}~\cite{principlesofdeeplearning-2022} (see Appendix A.2) which is bounded by a small constant. The dimension of the proposed MP problem is less than a few dozen; therefore, it can be solved by any off-the-shelf MP solver nearly instantly on the CPU. Deep-MAD requires NO GPU and NEVER creates deep models in memory. This makes Deep-MAD lightning fast even on CPU-only servers with small memory footprints. After solving the MP problem, the mathematically optimal CNN architecture is derived from the solution.

% Why we use the standard CNN block not more advanced ConvNext-block
Theoretically speaking, Deep-MAD is compatible with any CNN building blocks, including the aforementioned ViT-like ones. Yet this work aims to find a theoretically guided method to push the limitation of the old-school CNN to the next level without bells and whistles. This makes our work more challenging and more fundamental. Therefore, the remainder of this work will focus on the classic Conv+BN+ReLU ~\cite{si2015batchnorm,agarap2018deep} building block. In Section~\ref{section:verification_on_imagenet}, we also demonstrate that Deep-MAD is able to apply to modern building blocks such as depth-wise convolution~\cite{howard2017mobilenets, efficientnet} and SE module~\cite{hu2018squeeze}.

The contributions of our work are summarized as follows:
\begin{compactitem}
\item 
We propose Deep-MAD, a Mathematical Architecture Design paradigm for CNN architecture design backed up by modern deep learning theories.
\item We show that a high-performance CNN architecture can be derived from a constrained mathematical programming problem, which maximizes the differential entropy of the network \todo{with constrained effectiveness}.
\item
Deep-MAD achieves state-of-the-art performances in multiple large-scale vision datasets. Notably, Deep-MAD achieves 82.5\% top-1 accuracy on ImageNet-1k with 4.5 GFLOPs and 29M Params, outperforming ConvNeXt-Tiny (82.1\%) and Swin-Tiny (81.3\%) at the same scale.
\end{compactitem}
%------------------------------------------------------
